Trustworthiness-Driven Graph Convolutional Networks for Signed Network Embedding

The problem of representing nodes in a signed network as low-dimensional vectors, known as signed network embedding (SNE), has garnered considerable attention in recent years. While several SNE methods based on graph convolutional networks (GCN) have been proposed for this problem, we point out that they significantly rely on the assumption that the decades-old balance theory always holds in the real-world. To address this limitation, we propose a novel GCN-based SNE approach, named as TrustSGCN, which corrects for incorrect embedding propagation in GCN by utilizing the trustworthiness on edge signs for high-order relationships inferred by the balance theory. The proposed approach consists of three modules: (M1) generation of each node's extended ego-network; (M2) measurement of trustworthiness on edge signs; and (M3) trustworthiness-aware propagation of embeddings. Furthermore, TrustSGCN learns the node embeddings by leveraging two well-known societal theories, i.e., balance and status. The experiments on four real-world signed network datasets demonstrate that TrustSGCN consistently outperforms five state-of-the-art GCN-based SNE methods. The code is available at https://github.com/kmj0792/TrustSGCN.

==> table-eq4.tex <==
\begin{table*}[!t]
\footnotesize
\centering
\vspace{-0.0cm}
\caption{Sign prediction accuracies of two types of \ours\ with only sign loss and with both sign and status loss}
\vspace{-0.25cm}
\label{table:eq4}
\resizebox{\textwidth}{!} {
 \renewcommand{\arraystretch}{1}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}} & \multicolumn{3}{c|}{\textbf{Bitcoin-Alpha}} & \multicolumn{3}{c|}{\textbf{Bitcoin-OTC}}  & \multicolumn{3}{c|}{\textbf{Slashdot}} & \multicolumn{3}{c}{\textbf{Epinions}} \\ 
 & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{AUC} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{AUC} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{AUC} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{AUC} \\ \midrule

\textbf{$L_{sign}$} & 0.917 & 0.705 & 0.861 & 0.895 & 0.762 & 0.881 & 0.889 & 0.750 & 0.904 & 0.810 & 0.890 & 0.960  \\ 

\textbf{$L_{sign} + L_{status}$} &  \bf{0.921} & \bf{0.721} & \bf{0.867} & \bf{0.901} & \bf{0.773} & {\bf 0.886} & \bf{0.891} & \bf{0.765} & \bf{0.907} & \bf{0.920} & \bf{0.902} & \bf{0.966}  \\ 

\bottomrule
\end{tabular}
}
\vspace{-0.35cm}
\end{table*}

